Data Scaling Laws in NMT: The Effect of Noise and Architecture

In this work, we study the effect of varying the architecture and training data quality on the data scaling properties of Neural Machine Translation (NMT). First, we establish that the test loss of encoder-decoder transformer models scales as a power law in the number of training samples, with a dependence on the model size. Then, we systematically vary aspects of the training setup to understand how they impact the data scaling laws. In particular, we change the following (1) Architecture and task setup: We compare to a transformer-LSTM hybrid, and a decoder-only transformer with a language modeling loss (2) Noise level in the training distribution: We experiment with filtering, and adding iid synthetic noise. In all the above cases, we find that the data scaling exponents are minimally impacted, suggesting that marginally worse architectures or training data can be compensated for by adding more data. Lastly, we find that using back-translated data instead of parallel data, can significantly degrade the scaling exponent.

==> intro.tex <==
In deep learning, a reliable recipe to improve the generalization performance of a deep network is to increase the amount of compute and data used to train a model \citep{krizhevsky2012imagenet, brown2020language, radford2021learning}. Recent work \citep{kaplan2020scaling, rosenfeld2019constructive, Hestness2017DeepLS} has shown that these performance gains are not arbitrary --- the test performance of models, in fact, scales predictably as a power law in the various quantities of interest, such as the number of parameters ($N$), the number of training samples ($D$), and in the amount of compute ($C$) used for training. The precise reasons for why such scaling laws arise, and how different factors of the training setup (such as architecture, training distribution, noise etc) impact the scaling curves remains to be understood (see \citet{sharma2020neural, bahri2021explaining} for some potential explanations). A clearer understanding of the effect of different interventions to the training setup on the scaling laws can have several practical and theoretical benefits. In this work, we tackle this question for data scaling laws with the setup of neural machine translation (NMT):

\begin{center}
    \emph{Which changes to the training setup impact the data scaling co-efficients?}
\end{center}

% In addition to being an interesting phenomenon, these scaling laws can be leveraged for both practical and theoretical insights into deep learning.  %The existence of such scaling laws raises several interesting questions --- why do these scaling laws arise and which aspects of the training algorithm affect the scaling exponents of these scaling curves. 

Practically, data scaling laws can be leveraged to make experimental decisions for future larger scale experiments, and to decide where computational and research efforts should be focused. For instance, instead of comparing the performance of, say, two architectures at a single dataset size, we may want to compare their scaling exponents to better predict which architecture will perform better in the future as we gather more data.

\ynote{This part is rough}
Theoretically, the scaling of the test loss with respect to the dataset size can be considered as a ``signature" of the training setup (architecture and training method) that reveals how effectively a model leverages the data it is trained on. Hypothetically, if two architectures or two slightly different training distributions yield the same scaling exponent, this may be indicative of a deeper commonality in the mechanism by which these deep networks learn. For example, if we believe the model proposed by Sharma et. al. that deep networks essentially learn a d-dimensional manifold and perform 1-NN on this, then the exponent can tell us how a certain architecture represents the data.

\ynote{Maybe we should talk a bit about why *data* scaling - } \\
\ynote{We should also talk about benefits for NMT from this} \\
\orhanf{A. With the ever growing amounts of data the community has been using, especially for NLP models or neural models for text, is now reaching at the scales of the entire web.}\\
\orhanf{B. NMT models are trained using massive web-scale data, \citep{arivazhagan2019massively} used 25B training examples (~1T tokens) and with the invent of the techniques that confluence supervised + self-supervised learning \citep{liu2020multilingual,raffel2020exploring,siddhant2020leveraging} this number could easily reach to 10+T tokens.}

\bgh{An alternative to this line of discussion is the following: Our goal is to understand the sample efficiency of large-scale NMT models $->$ Because of this, we examine the data scaling laws for NMT $->$ and examine which interventions affect scaling laws significantly. NMT is a natural setting for performing such study because: (1) high quality bitext is hard to come by (2) Previous research (cite) has shown that composition bias of the data can severely affect the final performance of the model.}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/intro-summary-fig.png}
    \caption{\textbf{Data scaling exponent is minimally affected by changes to the training set up} (A) Changing the depth of the encoder-decoder transformer (B) Changing the architecture (C) Changing the noise in the training distribution \ynote{Describe details, add hybrids to B}}
    \label{fig:intro}
\end{figure}

\subsection{Our contributions}
We first show that the log-perplexity of encoder-decoder transformer models trained to perform neural machine translation (NMT) follows a power law in the dataset size, with a dependence on the model size (Figure \ref{fig:intro}A). We discuss some departures from prior work in the form of our scaling law, and demonstrate that our scaling law predicts experimental results over 3 orders of magnitude (from 500K-512M) training examples (sentence pairs in NMT) \footnote{Corresponding to ????? tokens}. Then, we systematically vary aspects of the training setup (listed below) to understand how these impact the scaling laws:


\begin{enumerate}
    \item {\bf Effect of architecture and loss:} We show that the scaling exponent for three different architectures (encoder-decoder transformers, decoder-only transformers and encoder transformer- decoder LSTM hybrids) is similar (Figure \ref{fig:intro}B). 
    \item {\bf Effect of data filtering:} We apply two common data filtering algorithms to our dataset and show that data filtering also manifests a multiplicative shift in the scaling curve. 
    \item {\bf Effect of synthetic noise:} We add iid synthetic noise (in the form of spelling errors, word deletions and sentence shuffling) to the source (input) and target (output) side separately and show that these types of noise also keep the scaling exponent constant (Figure \ref{fig:intro}C), but target noise can be more harmful than source noise.
    \item {\bf Effect of back-translated data:} We show that changing the training distribution to back-translated data does not impact the scaling exponent.
\end{enumerate}
\orhanf{1. Enumerated contributions part is a bit terse, we should revisit once the rest is done.}\\
\orhanf{2. I think it'll be nice to have a contribution explicitly stating ``practical recommendations" and have a subsection towards the end for that.}

Our work suggests that certain common operations used to boost performance, such as small changes to architecture or data filtering, can be replaced by adding an additional constant factor of data.

\subsection{Experimental Setup}
\label{sec:exp-setup}

\textbf{Models:} Our experiments are conducted on pre-layer transformer networks \citep{xiong2020layer}. Models are trained with per-token cross-entropy loss and Adafactor optimizer \citep{shazeer2018adafactor}. All models are trained with a fixed batch-size of 500K tokens and dropout rate of 0.1 for residuals, feed-forward activations and attention. For the small dataset sizes, the models are trained to early stopping (as measured on a held-out development set) and for large dataset sizes they are trained for up to 600K gradient steps.

The hyperparameters for these models were optimized for a 6 encoder layer and 6 decoder layer model trained on 2.2 billion sentence pairs.

\textbf{Training data} In our experiments, the models are trained on two large scale datasets. The first set of experiments on data size scaling are using the dataset sampled from an in-house parallel corpora containing up to 2.2B sentences translated from English to German. We sample training datasets of sizes \{1M, 2M, 4M, 8M, 16M, 32M, 64M, 128M, 256M, 512M\} independently to study the data scaling laws. The second set of experiments are conducted with Paracrawl dataset \citep{banon-etal-2020-paracrawl} and with added synthetic noise. The details are described in Section \ref{sec:noise}.

\textbf{Test data} The model performance is measured on a held-out dataset from the training distribution. Additionally, we also measure performance on various out-of-distribution test datasets. These test datasets have different domain composition and sampling methods. The domains considered are (i) Web-Domain (ii) News-Domain (iii) Wikipedia and (iv) Patents. The news-domain test sets come from the WMT2019 evaluation campaign (newstest2019) for all language pairs. The other test sets are internal test sets representing the different domains, ranging from 500 to 5000 sentence pairs for each set.
